Data-driven modeling for different stages of pandemic response

Some of the key questions of interest during the COVID-19 pandemic (and all outbreaks) include: where did the disease start, how is it spreading, who is at risk, and how to control the spread. There are a large number of complex factors driving the spread of pandemics, and, as a result, multiple modeling techniques play an increasingly important role in shaping public policy and decision making. As different countries and regions go through phases of the pandemic, the questions and data availability also changes. Especially of interest is aligning model development and data collection to support response efforts at each stage of the pandemic. The COVID-19 pandemic has been unprecedented in terms of real-time collection and dissemination of a number of diverse datasets, ranging from disease outcomes, to mobility, behaviors, and socio-economic factors. The data sets have been critical from the perspective of disease modeling and analytics to support policymakers in real-time. In this overview article, we survey the data landscape around COVID-19, with a focus on how such datasets have aided modeling and response through different stages so far in the pandemic. We also discuss some of the current challenges and the needs that will arise as we plan our way out of the pandemic.

==> Bios.tex <==
\section{Biographies}
\newlength\xL
\newlength\yL
\pgfmathsetlength{\xL}{0.13\textwidth}
\pgfmathsetlength{\yL}{0.12\textwidth}

\begin{wrapfigure}{r}{\xL}
\vspace{-13pt}
\centering
\includegraphics[width=\yL]{figs/aniruddha_adiga.jpg}
\end{wrapfigure}
Aniruddha Adiga is a Postdoctoral Research Associate at the NSSAC Division of the Biocomplexity Institute and initiative. He completed his PhD from the Department of Electrical Engineering, Indian Institute of Science (IISc), Bangalore, India and has held the position of Postdoctoral fellow at IISc and North Carolina State University, Raleigh, USA. 
His research areas include signal processing, machine learning, data mining, forecasting, big data analysis etc. At NSSAC, his primary focus has been the analysis and development of forecasting systems for epidemiological signals such as influenza-like illness and COVID-19 using auxiliary data sources.\medskip

\begin{wrapfigure}{l}{\xL}
\vspace{-13pt}
\centering\includegraphics[width=\yL]{figs/Jiangzhuo.jpg}
\end{wrapfigure}
Jiangzhuo Chen is a research associate professor in the Biocomplexity Institute, University of Virginia. He received his PhD in Computer Science from Northeastern University, and held positions at Virginia Tech before joining UVA. He has more than 10 years of experience in designing and implementing high performance computational models for large scale socio-technical systems. He has co-developed three agent based large scale simulation tools, which have been used in many studies to support modeling, forecasting, and impact analysis for infectious diseases including Influenza, Ebola, and COVID-19. His current research interests include agent based modeling, computational epidemiology, and theory guided machine learning.
\medskip

\begin{wrapfigure}{r}{\xL}
\vspace{-13pt}
\centering\includegraphics[width=\yL]{figs/Madhav-Picture-Feb2019.pdf}
\end{wrapfigure}
Madhav Marathe is a Distinguished Professor in 
Biocomplexity, the division director of the Networks, Simulation Science and Advanced Computing Division at the Biocomplexity Institute and Initiative, and a Professor in the Department of Computer Science at the University of Virginia (UVA). His research interests are in network science, computational epidemiology, AI, foundations of computing, socially coupled system science and high performance computing. Before joining UVA, he held positions at Virginia Tech and  the Los Alamos National Laboratory. He is a Fellow of the IEEE, ACM, SIAM and AAAS.\medskip



\begin{wrapfigure}{l}{\xL}
\vspace{-13pt}
\centering\includegraphics[width=\yL]{figs/Henning.jpg}
\end{wrapfigure}
Henning Mortveit is an associate professor with joint appointments at the Networks, Simulation Science and Advanced Computing Division at the Biocomplexity Institute and Initiative, and at the Department of Systems Engineering and Environment at the University of Virginia (UVA). His research is focused on massively interacting systems (MIS), their mathematical theory as captured through graph dynamical system, modeling and simulation science for MIS, as well as supporting system \& architecture design for scientifically reproducible, high performance simulation science of MIS. Before joining UVA, he held positions at Virginia Tech and at the Los Alamos National Laboratory.\medskip

\begin{wrapfigure}{r}{\xL}
\vspace{-13pt}
\centering\includegraphics[width=\yL]{figs/Srini_Headshot_2019.jpg}
\end{wrapfigure}
Srinivasan (Srini) Venkatramanan is a Research Scientist at the Biocomplexity Institute \& Initiative, University of Virginia and his research focuses on developing, analyzing and optimizing computational models in the field of network epidemiology. He received his PhD from the Department of Electrical and Communication Engineering, Indian Institute of Science (IISc), and did his postdoctoral research at Virginia Tech. His areas of interest include network science, stochastic modeling and big data analytics. He has used in-silico models of society to study the spread of infectious diseases and invasive species. Recent research includes modeling and forecasting emerging infectious disease outbreaks (e.g., Ebola, COVID-19), impact of human mobility on disease spread and resource allocation problems in the context of epidemic control (e.g., seasonal influenza vaccines). \medskip


\begin{wrapfigure}{l}{\xL}
\vspace{-13pt}
\centering\includegraphics[width=\yL]{figs/anil.jpg}
\end{wrapfigure}
Anil Vullikanti is a Professor in the Biocomplexity Institute and the Department of Computer Science
at the University of Virginia. He got his PhD at the Indian Institute of Science, and was a postdoctoral associate at the Max Planck Institute for Computer Science, Saarbr\"ucken, Germany, and the Los Alamos National Lab. His research interests are in the broad areas of network science, dynamical systems, combinatorial optimization, and distributed computing, and their applications to computational epidemiology and social networks.

==> old-background.tex <==

\section{Background}
\label{sec:models}

The modeling and analysis of epidemics has a long history; see, e.g.,
~\cite{anderson+m:book,marathe:cacm13,newman:sirev,brauer2001mathematical,castillo2013mathematical}. 
The most basic such models are of the SIR-type (see, e.g., ~\cite{newman:sirev, marathe:cacm13, anderson+m:book} for details). They capture a population as $n$ \emph{agents}, divided into three states: susceptible ($S$), infectious ($I$) and removed or recovered ($R$).  The particular model then specifies how susceptible individuals become infectious, and then recover. In its simplest form, the population is assumed to be mixed and  the dynamics of disease is described by a system of coupled ordinary differential equations.  Unfortunately, such mechanistic models of disease spread are usually too simplistic. Significant amount of research has been conducted to extend the model, usually in two broad ways \cite{barrett:wsc09, halloran:pnas08, eubank:nature04, ajelli:agbchrmv-2010,
epi:worldwide, ferguson:nature07}. 

The first involves structured meta-population models, which construct an abstraction of the mixing patterns in the population into different sub-populations, e.g., within smaller geographical regions, which are connected through airline and commuter flow networks~\cite{balcan:pnas2009, srini:ploscb19, zhang:pnas17, chinazzi:science20}. Such models are very useful in  the early days of an outbreak, when the disease dynamics are
largely driven by mobility and there is significant uncertainty in the (disease model) parameters. However, once the outbreak has spread, these models become less useful since it is difficult to integrate the effects of  detailed interventions
(e.g., social distancing) into the model. 

Due to these drawbacks of meta-population models, another approach using \emph{agent-based models}, are more useful, particularly after the outbreak.
Such models represent complex disease evolution and behavioral responses at the level of individual agents---these are typically humans, but can be animals, or other entities, such as organizations, in general. Such a model can be represented as a networked dynamical system, defined on a 
contact network $G(V,E)$ 
on a population $V$. where each edge $e=(u,v)\in E$ implies that
individuals (also referred to as nodes) $u, v\in V$ come into contact.
The SIR model on the graph $G$ is a dynamical process in which
each node is in one of $S$, $I$ or $R$ states.  Infection can
potentially spread from $u$ to $v$ along edge $e=(u,v)$ with a probability of
$\beta(e,t)$ at time instant $t$
after $u$ becomes infected, conditional on node $v$ remaining uninfected
until time $t$. 
We let $I(t)$ denote the set of nodes that become infected at time $t$. There can be additional staes, depending on the disease. For instance, COVID-19 requires modeling exposed and asymptomatic states, as well as states capturing hospitalization.

\begin{figure*}
\begin{center}
\includegraphics[width=0.75\linewidth]{figs/sir2.jpg}
%\vspace{-0.23in}
\caption{The SIR process on a graph. The contact graph $G=(V, E)$ is defined on
a population $V=\{1, 2, 3, 4\}$. The node colors yellow, red and green represent
the Susceptible, Infected and Recovered states, respectively. Initially, only node $1$ is infected, and all other nodes are susceptible. A possible outcome at $t=1$
is shown, in which node $3$ becomes infected, while node $1$ recovers. Node $1$ tries
to independently infect both its neighbors $2$ and $3$, but only node $3$ gets
infected--- this is indicated by the solid edge $(a, c)$.
The probability of getting
this outcome is $(1-p(1,2))p(1,3)$.
The configuration at $t=3$ is a ``fixed point''.
}
\label{fig:network-ex}
\end{center}
\end{figure*}


Figure~\ref{fig:network-ex} shows an example of the SIR model on a network $G=(V, E)$, and the dynamics of the SIR process.
In general, the graph $G$ is temporal and dynamic: the edge $e_t=(u, v)$ represents a contact between the nodes $u$ and $v$ at some time $t$. The network evolves at a similar time scale as the disease.
Further, each node and edge has attributes. Node attributes include demographic factors, e.g., age and gender, while edge attributes specify the type of activity when contact happened, and the duration of contact.
Further, the networks are multi-layer and heterogeneous graphs---nodes could be in different types and are often connected by multi-typed edges. 
%the specific contagion process might be different at each level








